Enhanced Marginal Sensitivity Model and Bounds

Sensitivity analysis is important to assess the impact of unmeasured confounding in causal inference from observational studies. The marginal sensitivity model (MSM) provides a useful approach in quantifying the influence of unmeasured confounders on treatment assignment and leading to tractable sharp bounds of common causal parameters. In this paper, to tighten MSM sharp bounds, we propose the enhanced MSM (eMSM) by incorporating another sensitivity constraint that quantifies the influence of unmeasured confounders on outcomes. We derive sharp population bounds of expected potential outcomes under eMSM, which are always narrower than the MSM sharp bounds in a simple and interpretable way. We further discuss desirable specifications of sensitivity parameters related to the outcome sensitivity constraint, and obtain both doubly robust point estimation and confidence intervals for the eMSM population bounds. The effectiveness of eMSM is also demonstrated numerically through two real-data applications. Our development represents, for the first time, a satisfactory extension of MSM to exploit both treatment and outcome sensitivity constraints on unmeasured confounding.

==> supp3.tex <==
We provide additional results for the empirical applications to RHC and NHANES.

\subsection{Additional numerical result for RHC} \label{sec:additional-numerical-rhc}
Figure \ref{fig:rhc-lowdim-logit-mu} presents the point bounds and 90\% confidence intervals on 30-day survival probabilities, similarly as Figure \ref{fig:rhc-lowdim-logit-ate}.
Figure \ref{fig:rhc-lowdim-lin} presents the point bounds and 90\% confidence intervals using working models with only main effects and linear outcome mean regression for CAL under MSM and eMSM. Figures \ref{fig:rhc-highdim-logit} and \ref{fig:rhc-highdim-lin} present the point bounds and 90\% confidence intervals using working models with main effects and interactions, with logistic and linear outcome mean regression applied to RCAL under MSM and eMSM, respectively. Tables \ref{tb:rhc-lowdim-cal-lam1.0}--\ref{tb:rhc-lowdim-dv-lam2.0} show the numerical estimates and standard errors using working models with only main effects. Tables \ref{tb:rhc-highdim-cal-lam1.0}--\ref{tb:rhc-highdim-cal-lam2.0} show the numerical estimates and standard errors using workings models with main effects and interactions.

Comparing Figures \ref{fig:rhc-lowdim-logit-ate} and \ref{fig:rhc-lowdim-lin}, we find that the conclusions in Section \ref{sec:rhc} remain valid for CAL under MSM and eMSM when using working models with linear outcome mean regression. By comparing numerical estimates and standard errors between the low-dimensional setting (Tables \ref{tb:rhc-lowdim-cal-lam1.0}–\ref{tb:rhc-lowdim-dv-lam2.0}) and the high-dimensional setting (Tables \ref{tb:rhc-highdim-cal-lam1.0}–\ref{tb:rhc-highdim-cal-lam2.0}), we observe that, in the high-dimensional setting, the point bounds for ATE are overall similar, while the standard errors of the point bounds are consistently smaller due to regularized estimation with more flexible working models, as observed in Tan (2024a).


\begin{figure}[h]
    \centering
    % First row: Lambda = 1
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-logit-mu-lam1.0.eps} \vspace{-.4in}
        \subcaption{ \small $\Lambda = 1$}
    \end{minipage}
    \hfill
    % First row: Lambda = 1.2
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-logit-mu-lam1.2.eps} \vspace{-.4in}
        \subcaption{\small $\Lambda = 1.2$}
    \end{minipage}
    
    \vspace{0.3in} % Add space between rows

    % Second row: Lambda = 1.5
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-logit-mu-lam1.5.eps} \vspace{-.4in}
        \subcaption{\small $\Lambda = 1.5$}
    \end{minipage}
    \hfill
    % Second row: Lambda = 2
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-logit-mu-lam2.0.eps} \vspace{-.4in}
        \subcaption{\small $\Lambda = 2$}
    \end{minipage} \vspace{-.1in}

    \caption{\small
Point bounds (x) and 90\% confidence intervals (–) on 30-day survival probabilities in the RHC study, similarly as Figure \ref{fig:rhc-lowdim-logit-ate}.}
    \label{fig:rhc-lowdim-logit-mu}
\end{figure}


\begin{figure} 
\centering
\begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-lin-lam1.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1$}
    \end{minipage}
    
    \vspace{.3in}
    
  \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-lin-lam1.2.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.2$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-lin-lam1.5.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.5$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-lowdim-lin-lam2.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 2$}
    \end{minipage} \vspace{-.1in}
\caption{\small
Point bounds (x) and 90\% confidence intervals (–) on 30-day survival probabilities, ATE and CRR in the RHC study, similarly as Figure \ref{fig:rhc-lowdim-logit-ate}, but using linear outcome mean regression for CAL under MSM and eMSM.}
\label{fig:rhc-lowdim-lin}
\end{figure}


\begin{figure} 
\centering
\begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-logit-lam1.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1$}
    \end{minipage}
    
    \vspace{.3in}
    
  \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-logit-lam1.2.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.2$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-logit-lam1.5.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.5$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-logit-lam2.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 2$}
    \end{minipage} \vspace{-.1in}
\caption{\small
Point bounds (x) and 90\% confidence intervals (–) on 30-day survival probabilities, ATE and CRR in the RHC study, similarly as Figure \ref{fig:rhc-lowdim-logit-ate}, but using working models with main effects and interactions.}
\label{fig:rhc-highdim-logit}
\end{figure}


\begin{figure} 
\centering
\begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-lin-lam1.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1$}
    \end{minipage}
    
    \vspace{.3in}
    
  \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-lin-lam1.2.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.2$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-lin-lam1.5.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 1.5$}
    \end{minipage}
    
    \vspace{.3in}
    
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rhc-highdim-lin-lam2.0.eps} \vspace{-.4in}
        \subcaption{$\Lambda = 2$}
    \end{minipage} \vspace{-.1in}
\caption{\small
Point bounds (x) and 90\% confidence intervals (–) on 30-day survival probabilities, ATE and CRR in the RHC study, similarly as Figure \ref{fig:rhc-highdim-logit}, but using linear outcome mean regression for RCAL under MSM and eMSM.}
\label{fig:rhc-highdim-lin}
\end{figure}

\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 1$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-cal-lam1.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012\\
MSM lin &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013\\
eMSM logit &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012\\
eMSM lin &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012\\
MSM lin &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013\\
eMSM logit &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012 &  &  0.634 &  0.012\\
eMSM lin &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013 &  &  0.635 &  0.013\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008\\
MSM lin &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008\\
eMSM logit &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008\\
eMSM lin &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008\\
MSM lin &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008\\
eMSM logit &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008 &  &  0.693 &  0.008\\
eMSM lin &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008 &  &  0.692 &  0.008\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014\\
MSM lin &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015\\
eMSM logit &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014\\
eMSM lin &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014\\
MSM lin &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015\\
eMSM logit &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014 &  &  -0.059 &   0.014\\
eMSM lin &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015 &  &  -0.058 &   0.015\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020\\
MSM lin &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021\\
eMSM logit &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020\\
eMSM lin &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020\\
MSM lin &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021\\
eMSM logit &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020 &  &  0.915 &  0.020\\
eMSM lin &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021 &  &  0.916 &  0.021\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote CAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for DV method under DV model with $\Lambda = 1$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-dv-lam1.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.625 &  0.013 &  &  0.625 &  0.013 &  &  0.625 &  0.013\\
DV $\Theta^+$ &  0.625 &  0.013 &  &  0.625 &  0.013 &  &  0.625 &  0.013 &  &  0.625 &  0.013\\
DV $3\Theta^+/2$ &  0.625 &  0.013 &  &  0.625 &  0.013 &  &  0.625 &  0.013 &  &  0.625 &  0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012\\
DV $\Theta^+$ &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012\\
DV $3\Theta^+/2$ &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012 &  &  0.625 &  0.012\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008\\
DV $\Theta^+$ &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008\\
DV $3\Theta^+/2$ &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008 &  &  0.690 &  0.008\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009\\
DV $\Theta^+$ &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009\\
DV $3\Theta^+/2$ &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009 &  &  0.690 &  0.009\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014\\
DV $\Theta^+$ &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014\\
DV $3\Theta^+/2$ &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014 &  &  -0.064 &   0.014\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015\\
DV $\Theta^+$ &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015\\
DV $3\Theta^+/2$ &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015 &  &  -0.064 &   0.015\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019\\
DV $\Theta^+$ &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019\\
DV $3\Theta^+/2$ &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019 &  &  0.907 &  0.019\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021\\
DV $\Theta^+$ &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021\\
DV $3\Theta^+/2$ &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021 &  &  0.907 &  0.021\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: DV $\Theta^+ / 2$,  DV $\Theta^+$ and DV $3\Theta^+ / 2$ denote DV method under DV model with $\Theta = \Theta^+ / 2$, $\Theta = \Theta^+$ and $\Theta = 3\Theta^+ / 2$. SEs for DV method are computed by matching the lower and upper points of the 90\% sensitivity interval with 
``lower point bound$- z_{0.05}$ SE'' and ``upper point bound$+ z_{0.05}$ SE'' respectively, where $z_{0.05}$ is the 95\% quantile of the standard normal distribution.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 1.2$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-cal-lam1.2} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.598 &  0.013 &  &  0.598 &  0.013 &  &  0.598 &  0.013 &  &  0.598 &  0.013\\
MSM lin &  0.601 &  0.014 &  &  0.601 &  0.014 &  &  0.601 &  0.014 &  &  0.601 &  0.014\\
eMSM logit &  0.626 &  0.013 &  &  0.616 &  0.013 &  &  0.605 &  0.013 &  &  0.598 &  0.013\\
eMSM lin &  0.628 &  0.013 &  &  0.618 &  0.013 &  &  0.608 &  0.014 &  &  0.601 &  0.014\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.665 &  0.012 &  &  0.665 &  0.012 &  &  0.665 &  0.012 &  &  0.665 &  0.012\\
MSM lin &  0.664 &  0.012 &  &  0.664 &  0.012 &  &  0.664 &  0.012 &  &  0.664 &  0.012\\
eMSM logit &  0.640 &  0.012 &  &  0.649 &  0.012 &  &  0.659 &  0.012 &  &  0.665 &  0.012\\
eMSM lin &  0.640 &  0.013 &  &  0.649 &  0.012 &  &  0.658 &  0.012 &  &  0.664 &  0.012\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.672 &  0.009 &  &  0.672 &  0.009 &  &  0.672 &  0.009 &  &  0.672 &  0.009\\
MSM lin &  0.672 &  0.009 &  &  0.672 &  0.009 &  &  0.672 &  0.009 &  &  0.672 &  0.009\\
eMSM logit &  0.689 &  0.008 &  &  0.683 &  0.008 &  &  0.676 &  0.008 &  &  0.672 &  0.009\\
eMSM lin &  0.688 &  0.008 &  &  0.682 &  0.008 &  &  0.676 &  0.009 &  &  0.672 &  0.009\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.711 &  0.008 &  &  0.711 &  0.008 &  &  0.711 &  0.008 &  &  0.711 &  0.008\\
MSM lin &  0.711 &  0.008 &  &  0.711 &  0.008 &  &  0.711 &  0.008 &  &  0.711 &  0.008\\
eMSM logit &  0.696 &  0.008 &  &  0.702 &  0.008 &  &  0.707 &  0.008 &  &  0.711 &  0.008\\
eMSM lin &  0.696 &  0.008 &  &  0.701 &  0.008 &  &  0.707 &  0.008 &  &  0.711 &  0.008\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.113 &   0.015 &  &  -0.113 &   0.015 &  &  -0.113 &   0.015 &  &  -0.113 &   0.015\\
MSM lin &  -0.110 &   0.015 &  &  -0.110 &   0.015 &  &  -0.110 &   0.015 &  &  -0.110 &   0.015\\
eMSM logit &  -0.070 &   0.014 &  &  -0.086 &   0.015 &  &  -0.102 &   0.015 &  &  -0.113 &   0.015\\
eMSM lin &  -0.068 &   0.015 &  &  -0.084 &   0.015 &  &  -0.099 &   0.015 &  &  -0.110 &   0.015\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.007 &   0.014 &  &  -0.007 &   0.014 &  &  -0.007 &   0.014 &  &  -0.007 &   0.014\\
MSM lin &  -0.008 &   0.014 &  &  -0.008 &   0.014 &  &  -0.008 &   0.014 &  &  -0.008 &   0.014\\
eMSM logit &  -0.049 &   0.014 &  &  -0.033 &   0.014 &  &  -0.018 &   0.014 &  &  -0.007 &   0.014\\
eMSM lin &  -0.048 &   0.014 &  &  -0.033 &   0.014 &  &  -0.018 &   0.014 &  &  -0.008 &   0.014\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.841 &  0.020 &  &  0.841 &  0.020 &  &  0.841 &  0.020 &  &  0.841 &  0.020\\
MSM lin &  0.846 &  0.021 &  &  0.846 &  0.021 &  &  0.846 &  0.021 &  &  0.846 &  0.021\\
eMSM logit &  0.900 &  0.020 &  &  0.878 &  0.020 &  &  0.856 &  0.020 &  &  0.841 &  0.020\\
eMSM lin &  0.902 &  0.021 &  &  0.881 &  0.021 &  &  0.860 &  0.021 &  &  0.846 &  0.021\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.989 &  0.021 &  &  0.989 &  0.021 &  &  0.989 &  0.021 &  &  0.989 &  0.021\\
MSM lin &  0.988 &  0.021 &  &  0.988 &  0.021 &  &  0.988 &  0.021 &  &  0.988 &  0.021\\
eMSM logit &  0.929 &  0.020 &  &  0.951 &  0.020 &  &  0.974 &  0.020 &  &  0.989 &  0.021\\
eMSM lin &  0.930 &  0.021 &  &  0.952 &  0.021 &  &  0.973 &  0.021 &  &  0.988 &  0.021\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote CAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}



\begin{table}
\caption{\footnotesize Point bounds and SEs for DV method under DV model with $\Lambda = 1.2$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-dv-lam1.2} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.601 &  0.012 &  &  0.574 &  0.011 &  &  0.560 &  0.011\\
DV $\Theta^+$ &  0.602 &  0.012 &  &  0.581 &  0.011 &  &  0.567 &  0.011 &  &  0.560 &  0.011\\
DV $3\Theta^+/2$ &  0.588 &  0.012 &  &  0.574 &  0.011 &  &  0.565 &  0.011 &  &  0.560 &  0.011\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.651 &  0.013 &  &  0.685 &  0.014 &  &  0.703 &  0.014\\
DV $\Theta^+$ &  0.650 &  0.013 &  &  0.676 &  0.013 &  &  0.694 &  0.014 &  &  0.703 &  0.014\\
DV $3\Theta^+/2$ &  0.666 &  0.013 &  &  0.684 &  0.014 &  &  0.697 &  0.014 &  &  0.703 &  0.014\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.008 &  &  0.673 &  0.008 &  &  0.655 &  0.007 &  &  0.646 &  0.007\\
DV $\Theta^+$ &  0.674 &  0.008 &  &  0.660 &  0.007 &  &  0.651 &  0.007 &  &  0.646 &  0.007\\
DV $3\Theta^+/2$ &  0.665 &  0.007 &  &  0.655 &  0.007 &  &  0.649 &  0.007 &  &  0.646 &  0.007\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.009 &  &  0.707 &  0.009 &  &  0.729 &  0.009 &  &  0.742 &  0.009\\
DV $\Theta^+$ &  0.706 &  0.009 &  &  0.723 &  0.009 &  &  0.735 &  0.009 &  &  0.742 &  0.009\\
DV $3\Theta^+/2$ &  0.717 &  0.009 &  &  0.729 &  0.009 &  &  0.737 &  0.009 &  &  0.742 &  0.009\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.014 &  &  -0.106 &   0.013 &  &  -0.156 &   0.013 &  &  -0.181 &   0.013\\
DV $\Theta^+$ &  -0.104 &   0.013 &  &  -0.143 &   0.013 &  &  -0.168 &   0.013 &  &  -0.181 &   0.013\\
DV $3\Theta^+/2$ &  -0.129 &   0.013 &  &  -0.155 &   0.013 &  &  -0.173 &   0.013 &  &  -0.181 &   0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.015 &  &  -0.022 &   0.015 &  &   0.030 &   0.015 &  &   0.057 &   0.016\\
DV $\Theta^+$ &  -0.025 &   0.015 &  &   0.016 &   0.015 &  &   0.043 &   0.016 &  &   0.057 &   0.016\\
DV $3\Theta^+/2$ &   0.001 &   0.015 &  &   0.029 &   0.015 &  &   0.048 &   0.016 &  &   0.057 &   0.016\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.019 &  &  0.850 &  0.018 &  &  0.786 &  0.017 &  &  0.756 &  0.016\\
DV $\Theta^+$ &  0.853 &  0.018 &  &  0.803 &  0.017 &  &  0.771 &  0.016 &  &  0.756 &  0.016\\
DV $3\Theta^+/2$ &  0.821 &  0.017 &  &  0.787 &  0.017 &  &  0.766 &  0.016 &  &  0.756 &  0.016\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.021 &  &  0.967 &  0.022 &  &  1.045 &  0.024 &  &  1.088 &  0.025\\
DV $\Theta^+$ &  0.964 &  0.022 &  &  1.024 &  0.024 &  &  1.066 &  0.025 &  &  1.088 &  0.025\\
DV $3\Theta^+/2$ &  1.002 &  0.023 &  &  1.044 &  0.024 &  &  1.073 &  0.025 &  &  1.088 &  0.025\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: DV $\Theta^+ / 2$,  DV $\Theta^+$ and DV $3\Theta^+ / 2$ denote DV method under DV model with $\Theta = \Theta^+ / 2$, $\Theta = \Theta^+$ and $\Theta = 3\Theta^+ / 2$. SEs for DV method are computed by matching the lower and upper points of the 90\% sensitivity interval with 
``lower point bound$- z_{0.05}$ SE'' and ``upper point bound$+ z_{0.05}$ SE'' respectively, where $z_{0.05}$ is the 95\% quantile of the standard normal distribution.}
\vspace{-.2in}
\end{table}



\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 1.5$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-cal-lam1.5} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.550 &  0.015 &  &  0.550 &  0.015 &  &  0.550 &  0.015 &  &  0.550 &  0.015\\
MSM lin &  0.555 &  0.015 &  &  0.555 &  0.015 &  &  0.555 &  0.015 &  &  0.555 &  0.015\\
eMSM logit &  0.617 &  0.013 &  &  0.592 &  0.013 &  &  0.567 &  0.014 &  &  0.550 &  0.015\\
eMSM lin &  0.619 &  0.013 &  &  0.595 &  0.014 &  &  0.571 &  0.015 &  &  0.555 &  0.015\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.700 &  0.011 &  &  0.700 &  0.011 &  &  0.700 &  0.011 &  &  0.700 &  0.011\\
MSM lin &  0.696 &  0.012 &  &  0.696 &  0.012 &  &  0.696 &  0.012 &  &  0.696 &  0.012\\
eMSM logit &  0.647 &  0.012 &  &  0.667 &  0.012 &  &  0.687 &  0.011 &  &  0.700 &  0.011\\
eMSM lin &  0.647 &  0.012 &  &  0.666 &  0.012 &  &  0.684 &  0.012 &  &  0.696 &  0.012\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.645 &  0.009 &  &  0.645 &  0.009 &  &  0.645 &  0.009 &  &  0.645 &  0.009\\
MSM lin &  0.645 &  0.010 &  &  0.645 &  0.010 &  &  0.645 &  0.010 &  &  0.645 &  0.010\\
eMSM logit &  0.683 &  0.008 &  &  0.669 &  0.009 &  &  0.654 &  0.009 &  &  0.645 &  0.009\\
eMSM lin &  0.683 &  0.008 &  &  0.669 &  0.009 &  &  0.655 &  0.009 &  &  0.645 &  0.010\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.730 &  0.007 &  &  0.730 &  0.007 &  &  0.730 &  0.007 &  &  0.730 &  0.007\\
MSM lin &  0.730 &  0.007 &  &  0.730 &  0.007 &  &  0.730 &  0.007 &  &  0.730 &  0.007\\
eMSM logit &  0.700 &  0.008 &  &  0.711 &  0.008 &  &  0.723 &  0.007 &  &  0.730 &  0.007\\
eMSM lin &  0.700 &  0.008 &  &  0.711 &  0.008 &  &  0.723 &  0.007 &  &  0.730 &  0.007\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.180 &   0.016 &  &  -0.180 &   0.016 &  &  -0.180 &   0.016 &  &  -0.180 &   0.016\\
MSM lin &  -0.175 &   0.016 &  &  -0.175 &   0.016 &  &  -0.175 &   0.016 &  &  -0.175 &   0.016\\
eMSM logit &  -0.084 &   0.015 &  &  -0.120 &   0.015 &  &  -0.156 &   0.015 &  &  -0.180 &   0.016\\
eMSM lin &  -0.081 &   0.015 &  &  -0.117 &   0.015 &  &  -0.152 &   0.016 &  &  -0.175 &   0.016\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &   0.056 &   0.014 &  &   0.056 &   0.014 &  &   0.056 &   0.014 &  &   0.056 &   0.014\\
MSM lin &   0.051 &   0.015 &  &   0.051 &   0.015 &  &   0.051 &   0.015 &  &   0.051 &   0.015\\
eMSM logit &  -0.036 &   0.014 &  &  -0.002 &   0.014 &  &   0.033 &   0.014 &  &   0.056 &   0.014\\
eMSM lin &  -0.036 &   0.014 &  &  -0.003 &   0.014 &  &   0.029 &   0.014 &  &   0.051 &   0.015\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.753 &  0.021 &  &  0.753 &  0.021 &  &  0.753 &  0.021 &  &  0.753 &  0.021\\
MSM lin &  0.760 &  0.022 &  &  0.760 &  0.022 &  &  0.760 &  0.022 &  &  0.760 &  0.022\\
eMSM logit &  0.881 &  0.020 &  &  0.831 &  0.020 &  &  0.784 &  0.020 &  &  0.753 &  0.021\\
eMSM lin &  0.884 &  0.021 &  &  0.836 &  0.021 &  &  0.790 &  0.021 &  &  0.760 &  0.022\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  1.086 &  0.022 &  &  1.086 &  0.022 &  &  1.086 &  0.022 &  &  1.086 &  0.022\\
MSM lin &  1.079 &  0.023 &  &  1.079 &  0.023 &  &  1.079 &  0.023 &  &  1.079 &  0.023\\
eMSM logit &  0.947 &  0.020 &  &  0.997 &  0.021 &  &  1.050 &  0.022 &  &  1.086 &  0.022\\
eMSM lin &  0.947 &  0.021 &  &  0.995 &  0.021 &  &  1.045 &  0.022 &  &  1.079 &  0.023\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote CAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}



\begin{table}
\caption{\footnotesize Point bounds and SEs for DV method under DV model with $\Lambda = 1.5$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-dv-lam1.5} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.570 &  0.011 &  &  0.519 &  0.010 &  &  0.495 &  0.009\\
DV $\Theta^+$ &  0.575 &  0.011 &  &  0.533 &  0.010 &  &  0.507 &  0.010 &  &  0.495 &  0.009\\
DV $3\Theta^+/2$ &  0.549 &  0.010 &  &  0.520 &  0.010 &  &  0.503 &  0.009 &  &  0.495 &  0.009\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.690 &  0.014 &  &  0.771 &  0.016 &  &  0.820 &  0.017\\
DV $\Theta^+$ &  0.682 &  0.014 &  &  0.747 &  0.015 &  &  0.794 &  0.017 &  &  0.820 &  0.017\\
DV $3\Theta^+/2$ &  0.720 &  0.015 &  &  0.769 &  0.016 &  &  0.803 &  0.017 &  &  0.820 &  0.017\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.008 &  &  0.652 &  0.007 &  &  0.619 &  0.007 &  &  0.603 &  0.007\\
DV $\Theta^+$ &  0.656 &  0.007 &  &  0.628 &  0.007 &  &  0.611 &  0.007 &  &  0.603 &  0.007\\
DV $3\Theta^+/2$ &  0.639 &  0.007 &  &  0.619 &  0.007 &  &  0.608 &  0.007 &  &  0.603 &  0.007\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.009 &  &  0.733 &  0.009 &  &  0.787 &  0.011 &  &  0.820 &  0.011\\
DV $\Theta^+$ &  0.728 &  0.009 &  &  0.771 &  0.010 &  &  0.803 &  0.011 &  &  0.820 &  0.011\\
DV $3\Theta^+/2$ &  0.753 &  0.010 &  &  0.786 &  0.011 &  &  0.808 &  0.011 &  &  0.820 &  0.011\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.014 &  &  -0.163 &   0.013 &  &  -0.268 &   0.013 &  &  -0.324 &   0.013\\
DV $\Theta^+$ &  -0.153 &   0.013 &  &  -0.238 &   0.013 &  &  -0.295 &   0.013 &  &  -0.324 &   0.013\\
DV $3\Theta^+/2$ &  -0.205 &   0.013 &  &  -0.265 &   0.013 &  &  -0.305 &   0.013 &  &  -0.324 &   0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.015 &  &   0.038 &   0.016 &  &   0.152 &   0.017 &  &   0.217 &   0.018\\
DV $\Theta^+$ &   0.026 &   0.015 &  &   0.119 &   0.017 &  &   0.184 &   0.018 &  &   0.217 &   0.018\\
DV $3\Theta^+/2$ &   0.082 &   0.016 &  &   0.150 &   0.017 &  &   0.194 &   0.018 &  &   0.217 &   0.018\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.019 &  &  0.777 &  0.016 &  &  0.659 &  0.014 &  &  0.605 &  0.012\\
DV $\Theta^+$ &  0.790 &  0.017 &  &  0.691 &  0.014 &  &  0.632 &  0.013 &  &  0.605 &  0.012\\
DV $3\Theta^+/2$ &  0.728 &  0.015 &  &  0.662 &  0.014 &  &  0.623 &  0.013 &  &  0.605 &  0.012\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.021 &  &  1.058 &  0.024 &  &  1.246 &  0.030 &  &  1.360 &  0.033\\
DV $\Theta^+$ &  1.040 &  0.024 &  &  1.190 &  0.028 &  &  1.300 &  0.031 &  &  1.360 &  0.033\\
DV $3\Theta^+/2$ &  1.128 &  0.026 &  &  1.241 &  0.029 &  &  1.320 &  0.031 &  &  1.360 &  0.033\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: DV $\Theta^+ / 2$,  DV $\Theta^+$ and DV $3\Theta^+ / 2$ denote DV method under DV model with $\Theta = \Theta^+ / 2$, $\Theta = \Theta^+$ and $\Theta = 3\Theta^+ / 2$. SEs for DV method are computed by matching the lower and upper points of the 90\% sensitivity interval with 
``lower point bound$- z_{0.05}$ SE'' and ``upper point bound$+ z_{0.05}$ SE'' respectively, where $z_{0.05}$ is the 95\% quantile of the standard normal distribution.}
\vspace{-.2in}
\end{table}




\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 2$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-cal-lam2.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.481 &  0.014 &  &  0.481 &  0.014 &  &  0.481 &  0.014 &  &  0.481 &  0.014\\
MSM lin &  0.495 &  0.015 &  &  0.495 &  0.015 &  &  0.495 &  0.015 &  &  0.495 &  0.015\\
eMSM logit &  0.603 &  0.013 &  &  0.557 &  0.013 &  &  0.512 &  0.014 &  &  0.481 &  0.014\\
eMSM lin &  0.607 &  0.013 &  &  0.565 &  0.014 &  &  0.523 &  0.014 &  &  0.495 &  0.015\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.742 &  0.011 &  &  0.742 &  0.011 &  &  0.742 &  0.011 &  &  0.742 &  0.011\\
MSM lin &  0.734 &  0.013 &  &  0.734 &  0.013 &  &  0.734 &  0.013 &  &  0.734 &  0.013\\
eMSM logit &  0.655 &  0.012 &  &  0.688 &  0.012 &  &  0.720 &  0.011 &  &  0.742 &  0.011\\
eMSM lin &  0.654 &  0.012 &  &  0.684 &  0.012 &  &  0.714 &  0.012 &  &  0.734 &  0.013\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.603 &  0.010 &  &  0.603 &  0.010 &  &  0.603 &  0.010 &  &  0.603 &  0.010\\
MSM lin &  0.608 &  0.010 &  &  0.608 &  0.010 &  &  0.608 &  0.010 &  &  0.608 &  0.010\\
eMSM logit &  0.675 &  0.008 &  &  0.648 &  0.009 &  &  0.621 &  0.009 &  &  0.603 &  0.010\\
eMSM lin &  0.675 &  0.008 &  &  0.650 &  0.009 &  &  0.625 &  0.009 &  &  0.608 &  0.010\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.750 &  0.007 &  &  0.750 &  0.007 &  &  0.750 &  0.007 &  &  0.750 &  0.007\\
MSM lin &  0.751 &  0.007 &  &  0.751 &  0.007 &  &  0.751 &  0.007 &  &  0.751 &  0.007\\
eMSM logit &  0.704 &  0.008 &  &  0.721 &  0.007 &  &  0.739 &  0.007 &  &  0.750 &  0.007\\
eMSM lin &  0.704 &  0.008 &  &  0.722 &  0.007 &  &  0.739 &  0.007 &  &  0.751 &  0.007\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.269 &   0.015 &  &  -0.269 &   0.015 &  &  -0.269 &   0.015 &  &  -0.269 &   0.015\\
MSM lin &  -0.256 &   0.016 &  &  -0.256 &   0.016 &  &  -0.256 &   0.016 &  &  -0.256 &   0.016\\
eMSM logit &  -0.101 &   0.014 &  &  -0.164 &   0.015 &  &  -0.227 &   0.015 &  &  -0.269 &   0.015\\
eMSM lin &  -0.097 &   0.015 &  &  -0.157 &   0.015 &  &  -0.216 &   0.015 &  &  -0.256 &   0.016\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &   0.138 &   0.014 &  &   0.138 &   0.014 &  &   0.138 &   0.014 &  &   0.138 &   0.014\\
MSM lin &   0.127 &   0.015 &  &   0.127 &   0.015 &  &   0.127 &   0.015 &  &   0.127 &   0.015\\
eMSM logit &  -0.020 &   0.014 &  &   0.040 &   0.014 &  &   0.099 &   0.014 &  &   0.138 &   0.014\\
eMSM lin &  -0.021 &   0.014 &  &   0.034 &   0.015 &  &   0.090 &   0.015 &  &   0.127 &   0.015\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.642 &  0.019 &  &  0.642 &  0.019 &  &  0.642 &  0.019 &  &  0.642 &  0.019\\
MSM lin &  0.659 &  0.020 &  &  0.659 &  0.020 &  &  0.659 &  0.020 &  &  0.659 &  0.020\\
eMSM logit &  0.856 &  0.020 &  &  0.772 &  0.019 &  &  0.693 &  0.019 &  &  0.642 &  0.019\\
eMSM lin &  0.862 &  0.020 &  &  0.783 &  0.020 &  &  0.708 &  0.020 &  &  0.659 &  0.020\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  1.229 &  0.026 &  &  1.229 &  0.026 &  &  1.229 &  0.026 &  &  1.229 &  0.026\\
MSM lin &  1.208 &  0.027 &  &  1.208 &  0.027 &  &  1.208 &  0.027 &  &  1.208 &  0.027\\
eMSM logit &  0.971 &  0.021 &  &  1.061 &  0.022 &  &  1.159 &  0.024 &  &  1.229 &  0.026\\
eMSM lin &  0.969 &  0.021 &  &  1.053 &  0.023 &  &  1.144 &  0.025 &  &  1.208 &  0.027\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote CAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression. The upper or lower point of the 90\% sensitivity interval is calculated as ``upper point bound$ + z_{0.05}$ SE'' or ``lower point bound$ -  z_{0.05}$ SE'' respectively. For example, as mentioned in the main text, the upper interval point for $\mu^1 - \mu^0$ from eMSM logit at $(\Lambda = 2, \delta = 0.2)$ is $-0.020 +  z_{0.05}\times 0.014 \approx 0.0030$.}
\vspace{-.2in}
\end{table}



\begin{table}
\caption{\footnotesize Point bounds and SEs for DV method under DV model with $\Lambda = 2$, using working models with only main effects in the RHC study.} \label{tb:rhc-lowdim-dv-lam2.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.528 &  0.010 &  &  0.461 &  0.008 &  &  0.431 &  0.008\\
DV $\Theta^+$ &  0.542 &  0.010 &  &  0.479 &  0.009 &  &  0.446 &  0.008 &  &  0.431 &  0.008\\
DV $3\Theta^+/2$ &  0.505 &  0.009 &  &  0.463 &  0.008 &  &  0.441 &  0.008 &  &  0.431 &  0.008\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
DV $\Theta^+/2$ &  0.625 &  0.012 &  &  0.755 &  0.016 &  &  0.911 &  0.020 &  &  1.014 &  0.023\\
DV $\Theta^+$ &  0.731 &  0.015 &  &  0.859 &  0.019 &  &  0.959 &  0.021 &  &  1.014 &  0.023\\
DV $3\Theta^+/2$ &  0.800 &  0.017 &  &  0.903 &  0.020 &  &  0.976 &  0.022 &  &  1.014 &  0.023\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.008 &  &  0.625 &  0.007 &  &  0.580 &  0.007 &  &  0.560 &  0.007\\
DV $\Theta^+$ &  0.634 &  0.007 &  &  0.592 &  0.007 &  &  0.570 &  0.007 &  &  0.560 &  0.007\\
DV $3\Theta^+/2$ &  0.609 &  0.007 &  &  0.581 &  0.007 &  &  0.566 &  0.007 &  &  0.560 &  0.007\\
 & \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
DV $\Theta^+/2$ &  0.690 &  0.009 &  &  0.776 &  0.010 &  &  0.880 &  0.012 &  &  0.950 &  0.014\\
DV $\Theta^+$ &  0.761 &  0.010 &  &  0.846 &  0.012 &  &  0.912 &  0.013 &  &  0.950 &  0.014\\
DV $3\Theta^+/2$ &  0.806 &  0.011 &  &  0.875 &  0.012 &  &  0.924 &  0.013 &  &  0.950 &  0.014\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.014 &  &  -0.248 &   0.013 &  &  -0.420 &   0.014 &  &  -0.519 &   0.015\\
DV $\Theta^+$ &  -0.219 &   0.013 &  &  -0.366 &   0.013 &  &  -0.467 &   0.014 &  &  -0.519 &   0.015\\
DV $3\Theta^+/2$ &  -0.301 &   0.013 &  &  -0.412 &   0.014 &  &  -0.484 &   0.014 &  &  -0.519 &   0.015\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
DV $\Theta^+/2$ &  -0.064 &   0.015 &  &   0.130 &   0.017 &  &   0.331 &   0.020 &  &   0.455 &   0.023\\
DV $\Theta^+$ &   0.097 &   0.016 &  &   0.267 &   0.019 &  &   0.389 &   0.021 &  &   0.455 &   0.023\\
DV $3\Theta^+/2$ &   0.190 &   0.018 &  &   0.322 &   0.020 &  &   0.410 &   0.022 &  &   0.455 &   0.023\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.019 &  &  0.680 &  0.014 &  &  0.523 &  0.010 &  &  0.453 &  0.009\\
DV $\Theta^+$ &  0.712 &  0.015 &  &  0.567 &  0.011 &  &  0.488 &  0.010 &  &  0.453 &  0.009\\
DV $3\Theta^+/2$ &  0.626 &  0.013 &  &  0.529 &  0.011 &  &  0.477 &  0.009 &  &  0.453 &  0.009\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
DV $\Theta^+/2$ &  0.907 &  0.021 &  &  1.209 &  0.029 &  &  1.571 &  0.038 &  &  1.812 &  0.044\\
DV $\Theta^+$ &  1.154 &  0.027 &  &  1.450 &  0.035 &  &  1.683 &  0.040 &  &  1.812 &  0.044\\
DV $3\Theta^+/2$ &  1.313 &  0.031 &  &  1.554 &  0.037 &  &  1.724 &  0.042 &  &  1.812 &  0.044\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: DV $\Theta^+ / 2$,  DV $\Theta^+$ and DV $3\Theta^+ / 2$ denote DV method under DV model with $\Theta = \Theta^+ / 2$, $\Theta = \Theta^+$ and $\Theta = 3\Theta^+ / 2$. SEs for DV method are computed by matching the lower and upper points of the 90\% sensitivity interval with 
``lower point bound$- z_{0.05}$ SE'' and ``upper point bound$+ z_{0.05}$ SE'' respectively, where $z_{0.05}$ is the 95\% quantile of the standard normal distribution.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 1$, using working models with main effects and interactions in the RHC study.} \label{tb:rhc-highdim-cal-lam1.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
MSM lin &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
eMSM logit &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
eMSM lin &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
MSM lin &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
eMSM logit &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
eMSM lin &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011 &  &  0.636 &  0.011\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008\\
MSM lin &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008\\
eMSM logit &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008\\
eMSM lin &  0.688 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008\\
MSM lin &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008\\
eMSM logit &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008 &  &  0.688 &  0.008\\
eMSM lin &  0.688 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008 &  &  0.687 &  0.008\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
MSM lin &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
eMSM logit &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
eMSM lin &  -0.052 &   0.013 &  &  -0.051 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
MSM lin &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
eMSM logit &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
eMSM lin &  -0.052 &   0.013 &  &  -0.051 &   0.013 &  &  -0.052 &   0.013 &  &  -0.052 &   0.013\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.924 &  0.018 &  &  0.924 &  0.018 &  &  0.924 &  0.018 &  &  0.924 &  0.018\\
MSM lin &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018\\
eMSM logit &  0.924 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.924 &  0.018\\
eMSM lin &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.924 &  0.018 &  &  0.924 &  0.018 &  &  0.924 &  0.018 &  &  0.924 &  0.018\\
MSM lin &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018\\
eMSM logit &  0.924 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.924 &  0.018\\
eMSM lin &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018 &  &  0.925 &  0.018\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote RCAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 1.2$, using working models with main effects and interactions in the RHC study.} \label{tb:rhc-highdim-cal-lam1.2} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.600 &  0.012 &  &  0.600 &  0.012 &  &  0.600 &  0.012 &  &  0.600 &  0.012\\
MSM lin &  0.601 &  0.012 &  &  0.601 &  0.012 &  &  0.601 &  0.012 &  &  0.601 &  0.012\\
eMSM logit &  0.629 &  0.011 &  &  0.618 &  0.011 &  &  0.608 &  0.012 &  &  0.600 &  0.012\\
eMSM lin &  0.629 &  0.011 &  &  0.618 &  0.011 &  &  0.607 &  0.011 &  &  0.601 &  0.012\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.667 &  0.010 &  &  0.667 &  0.010 &  &  0.667 &  0.010 &  &  0.667 &  0.010\\
MSM lin &  0.666 &  0.010 &  &  0.666 &  0.010 &  &  0.666 &  0.010 &  &  0.666 &  0.010\\
eMSM logit &  0.642 &  0.011 &  &  0.652 &  0.010 &  &  0.661 &  0.010 &  &  0.667 &  0.010\\
eMSM lin &  0.642 &  0.011 &  &  0.651 &  0.010 &  &  0.660 &  0.010 &  &  0.666 &  0.010\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.668 &  0.008 &  &  0.668 &  0.008 &  &  0.668 &  0.008 &  &  0.668 &  0.008\\
MSM lin &  0.669 &  0.008 &  &  0.669 &  0.008 &  &  0.669 &  0.008 &  &  0.669 &  0.008\\
eMSM logit &  0.684 &  0.008 &  &  0.678 &  0.008 &  &  0.672 &  0.008 &  &  0.668 &  0.008\\
eMSM lin &  0.684 &  0.008 &  &  0.678 &  0.008 &  &  0.672 &  0.008 &  &  0.669 &  0.008\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.706 &  0.007 &  &  0.706 &  0.007 &  &  0.706 &  0.007 &  &  0.706 &  0.007\\
MSM lin &  0.706 &  0.007 &  &  0.706 &  0.007 &  &  0.706 &  0.007 &  &  0.706 &  0.007\\
eMSM logit &  0.691 &  0.008 &  &  0.697 &  0.008 &  &  0.702 &  0.008 &  &  0.706 &  0.007\\
eMSM lin &  0.691 &  0.008 &  &  0.696 &  0.008 &  &  0.702 &  0.008 &  &  0.706 &  0.007\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.106 &   0.013 &  &  -0.106 &   0.013 &  &  -0.106 &   0.013 &  &  -0.106 &   0.013\\
MSM lin &  -0.105 &   0.013 &  &  -0.105 &   0.013 &  &  -0.105 &   0.013 &  &  -0.105 &   0.013\\
eMSM logit &  -0.063 &   0.013 &  &  -0.079 &   0.013 &  &  -0.095 &   0.013 &  &  -0.106 &   0.013\\
eMSM lin &  -0.062 &   0.013 &  &  -0.078 &   0.013 &  &  -0.094 &   0.013 &  &  -0.105 &   0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.001 &   0.012 &  &  -0.001 &   0.012 &  &  -0.001 &   0.012 &  &  -0.001 &   0.012\\
MSM lin &  -0.003 &   0.012 &  &  -0.003 &   0.012 &  &  -0.003 &   0.012 &  &  -0.003 &   0.012\\
eMSM logit &  -0.042 &   0.013 &  &  -0.026 &   0.012 &  &  -0.012 &   0.012 &  &  -0.001 &   0.012\\
eMSM lin &  -0.042 &   0.013 &  &  -0.027 &   0.013 &  &  -0.012 &   0.012 &  &  -0.003 &   0.012\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.850 &  0.018 &  &  0.850 &  0.018 &  &  0.850 &  0.018 &  &  0.850 &  0.018\\
MSM lin &  0.851 &  0.018 &  &  0.851 &  0.018 &  &  0.851 &  0.018 &  &  0.851 &  0.018\\
eMSM logit &  0.909 &  0.018 &  &  0.886 &  0.018 &  &  0.865 &  0.018 &  &  0.850 &  0.018\\
eMSM lin &  0.910 &  0.018 &  &  0.888 &  0.018 &  &  0.865 &  0.018 &  &  0.851 &  0.018\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.998 &  0.018 &  &  0.998 &  0.018 &  &  0.998 &  0.018 &  &  0.998 &  0.018\\
MSM lin &  0.996 &  0.018 &  &  0.996 &  0.018 &  &  0.996 &  0.018 &  &  0.996 &  0.018\\
eMSM logit &  0.939 &  0.018 &  &  0.961 &  0.018 &  &  0.983 &  0.018 &  &  0.998 &  0.018\\
eMSM lin &  0.939 &  0.018 &  &  0.961 &  0.018 &  &  0.981 &  0.018 &  &  0.996 &  0.018\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote RCAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 1.5$, using working models with main effects and interactions in the RHC study.} \label{tb:rhc-highdim-cal-lam1.5} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.562 &  0.012 &  &  0.562 &  0.012 &  &  0.562 &  0.012 &  &  0.562 &  0.012\\
MSM lin &  0.567 &  0.012 &  &  0.567 &  0.012 &  &  0.567 &  0.012 &  &  0.567 &  0.012\\
eMSM logit &  0.621 &  0.011 &  &  0.600 &  0.011 &  &  0.577 &  0.012 &  &  0.562 &  0.012\\
eMSM lin &  0.622 &  0.011 &  &  0.602 &  0.011 &  &  0.581 &  0.012 &  &  0.567 &  0.012\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.700 &  0.009 &  &  0.700 &  0.009 &  &  0.700 &  0.009 &  &  0.700 &  0.009\\
MSM lin &  0.698 &  0.009 &  &  0.698 &  0.009 &  &  0.698 &  0.009 &  &  0.698 &  0.009\\
eMSM logit &  0.649 &  0.010 &  &  0.668 &  0.010 &  &  0.687 &  0.009 &  &  0.700 &  0.009\\
eMSM lin &  0.648 &  0.010 &  &  0.667 &  0.010 &  &  0.686 &  0.009 &  &  0.698 &  0.009\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.641 &  0.009 &  &  0.641 &  0.009 &  &  0.641 &  0.009 &  &  0.641 &  0.009\\
MSM lin &  0.642 &  0.009 &  &  0.642 &  0.009 &  &  0.642 &  0.009 &  &  0.642 &  0.009\\
eMSM logit &  0.678 &  0.008 &  &  0.664 &  0.008 &  &  0.650 &  0.009 &  &  0.641 &  0.009\\
eMSM lin &  0.678 &  0.008 &  &  0.664 &  0.008 &  &  0.651 &  0.009 &  &  0.642 &  0.009\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.729 &  0.007 &  &  0.729 &  0.007 &  &  0.729 &  0.007 &  &  0.729 &  0.007\\
MSM lin &  0.728 &  0.007 &  &  0.728 &  0.007 &  &  0.728 &  0.007 &  &  0.728 &  0.007\\
eMSM logit &  0.696 &  0.008 &  &  0.708 &  0.007 &  &  0.720 &  0.007 &  &  0.729 &  0.007\\
eMSM lin &  0.696 &  0.008 &  &  0.708 &  0.007 &  &  0.720 &  0.007 &  &  0.728 &  0.007\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.166 &   0.013 &  &  -0.166 &   0.013 &  &  -0.166 &   0.013 &  &  -0.166 &   0.013\\
MSM lin &  -0.162 &   0.013 &  &  -0.162 &   0.013 &  &  -0.162 &   0.013 &  &  -0.162 &   0.013\\
eMSM logit &  -0.075 &   0.013 &  &  -0.109 &   0.013 &  &  -0.143 &   0.013 &  &  -0.166 &   0.013\\
eMSM lin &  -0.074 &   0.013 &  &  -0.106 &   0.013 &  &  -0.140 &   0.013 &  &  -0.162 &   0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &   0.059 &   0.012 &  &   0.059 &   0.012 &  &   0.059 &   0.012 &  &   0.059 &   0.012\\
MSM lin &   0.056 &   0.012 &  &   0.056 &   0.012 &  &   0.056 &   0.012 &  &   0.056 &   0.012\\
eMSM logit &  -0.030 &   0.012 &  &   0.004 &   0.012 &  &   0.037 &   0.012 &  &   0.059 &   0.012\\
eMSM lin &  -0.030 &   0.012 &  &   0.003 &   0.012 &  &   0.035 &   0.012 &  &   0.056 &   0.012\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.772 &  0.018 &  &  0.772 &  0.018 &  &  0.772 &  0.018 &  &  0.772 &  0.018\\
MSM lin &  0.778 &  0.018 &  &  0.778 &  0.018 &  &  0.778 &  0.018 &  &  0.778 &  0.018\\
eMSM logit &  0.892 &  0.018 &  &  0.846 &  0.018 &  &  0.802 &  0.018 &  &  0.772 &  0.018\\
eMSM lin &  0.894 &  0.018 &  &  0.850 &  0.018 &  &  0.806 &  0.018 &  &  0.778 &  0.018\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  1.092 &  0.019 &  &  1.092 &  0.019 &  &  1.092 &  0.019 &  &  1.092 &  0.019\\
MSM lin &  1.087 &  0.020 &  &  1.087 &  0.020 &  &  1.087 &  0.020 &  &  1.087 &  0.020\\
eMSM logit &  0.956 &  0.018 &  &  1.006 &  0.019 &  &  1.058 &  0.019 &  &  1.092 &  0.019\\
eMSM lin &  0.956 &  0.018 &  &  1.004 &  0.019 &  &  1.053 &  0.019 &  &  1.087 &  0.020\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote RCAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 2$, using working models with main effects and interactions in the RHC study.} \label{tb:rhc-highdim-cal-lam2.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM logit &  0.489 &  0.013 &  &  0.489 &  0.013 &  &  0.489 &  0.013 &  &  0.489 &  0.013\\
MSM lin &  0.490 &  0.013 &  &  0.490 &  0.013 &  &  0.490 &  0.013 &  &  0.490 &  0.013\\
eMSM logit &  0.607 &  0.011 &  &  0.563 &  0.012 &  &  0.519 &  0.012 &  &  0.489 &  0.013\\
eMSM lin &  0.607 &  0.011 &  &  0.563 &  0.012 &  &  0.519 &  0.012 &  &  0.490 &  0.013\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM logit &  0.734 &  0.008 &  &  0.734 &  0.008 &  &  0.734 &  0.008 &  &  0.734 &  0.008\\
MSM lin &  0.730 &  0.008 &  &  0.730 &  0.008 &  &  0.730 &  0.008 &  &  0.730 &  0.008\\
eMSM logit &  0.656 &  0.010 &  &  0.685 &  0.009 &  &  0.715 &  0.009 &  &  0.734 &  0.008\\
eMSM lin &  0.655 &  0.010 &  &  0.683 &  0.009 &  &  0.711 &  0.009 &  &  0.730 &  0.008\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM logit &  0.599 &  0.009 &  &  0.599 &  0.009 &  &  0.599 &  0.009 &  &  0.599 &  0.009\\
MSM lin &  0.602 &  0.009 &  &  0.602 &  0.009 &  &  0.602 &  0.009 &  &  0.602 &  0.009\\
eMSM logit &  0.670 &  0.008 &  &  0.643 &  0.008 &  &  0.617 &  0.009 &  &  0.599 &  0.009\\
eMSM lin &  0.670 &  0.008 &  &  0.644 &  0.009 &  &  0.619 &  0.009 &  &  0.602 &  0.009\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM logit &  0.749 &  0.006 &  &  0.749 &  0.006 &  &  0.749 &  0.006 &  &  0.749 &  0.006\\
MSM lin &  0.749 &  0.006 &  &  0.749 &  0.006 &  &  0.749 &  0.006 &  &  0.749 &  0.006\\
eMSM logit &  0.700 &  0.008 &  &  0.718 &  0.007 &  &  0.737 &  0.007 &  &  0.749 &  0.006\\
eMSM lin &  0.699 &  0.008 &  &  0.718 &  0.007 &  &  0.736 &  0.007 &  &  0.749 &  0.006\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &  -0.260 &   0.014 &  &  -0.260 &   0.014 &  &  -0.260 &   0.014 &  &  -0.260 &   0.014\\
MSM lin &  -0.259 &   0.014 &  &  -0.259 &   0.014 &  &  -0.259 &   0.014 &  &  -0.259 &   0.014\\
eMSM logit &  -0.093 &   0.013 &  &  -0.156 &   0.013 &  &  -0.218 &   0.013 &  &  -0.260 &   0.014\\
eMSM lin &  -0.093 &   0.013 &  &  -0.155 &   0.013 &  &  -0.217 &   0.014 &  &  -0.259 &   0.014\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM logit &   0.135 &   0.011 &  &   0.135 &   0.011 &  &   0.135 &   0.011 &  &   0.135 &   0.011\\
MSM lin &   0.128 &   0.011 &  &   0.128 &   0.011 &  &   0.128 &   0.011 &  &   0.128 &   0.011\\
eMSM logit &  -0.014 &   0.012 &  &   0.042 &   0.012 &  &   0.098 &   0.012 &  &   0.135 &   0.011\\
eMSM lin &  -0.015 &   0.012 &  &   0.039 &   0.012 &  &   0.093 &   0.012 &  &   0.128 &   0.011\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  0.653 &  0.018 &  &  0.653 &  0.018 &  &  0.653 &  0.018 &  &  0.653 &  0.018\\
MSM lin &  0.655 &  0.018 &  &  0.655 &  0.018 &  &  0.655 &  0.018 &  &  0.655 &  0.018\\
eMSM logit &  0.867 &  0.018 &  &  0.783 &  0.017 &  &  0.704 &  0.017 &  &  0.653 &  0.018\\
eMSM lin &  0.868 &  0.018 &  &  0.784 &  0.017 &  &  0.706 &  0.018 &  &  0.655 &  0.018\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 / \mu^0$} \\
MSM logit &  1.226 &  0.022 &  &  1.226 &  0.022 &  &  1.226 &  0.022 &  &  1.226 &  0.022\\
MSM lin &  1.213 &  0.021 &  &  1.213 &  0.021 &  &  1.213 &  0.021 &  &  1.213 &  0.021\\
eMSM logit &  0.979 &  0.018 &  &  1.065 &  0.019 &  &  1.159 &  0.020 &  &  1.226 &  0.022\\
eMSM lin &  0.977 &  0.018 &  &  1.061 &  0.019 &  &  1.150 &  0.020 &  &  1.213 &  0.021\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM logit and eMSM logit denote RCAL under MSM and eMSM using logistic outcome mean regression. MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}







\subsection{Additional numerical result for NHANES} \label{sec:additional-numerical-nhanes}
Figure \ref{fig:nhanes-highdim-lin} presents the point bounds and 90\% confidence intervals on mean blood mercury and average treatment effect, similarly as Figure \ref{fig:nhanes-highdim-lin-ate}.
Figure \ref{fig:nhanes-lowdim-lin} presents the point bounds and 90\% confidence intervals using working models with only main effects and linear outcome mean regression for CAL under MSM and eMSM. Tables \ref{tb:nhanes-lowdim-cal-lam1.0}--\ref{tb:nhanes-lowdim-cal-lam50} show numerical estimates and standard errors using working models with only main effects and Tables \ref{tb:nhanes-highdim-cal-lam1.0}--\ref{tb:nhanes-highdim-cal-lam50} show numerical estimates and standard errors using working models with main effects and interactions.

Comparing Figures \ref{fig:nhanes-highdim-lin-ate} and \ref{fig:nhanes-lowdim-lin}, we see notable differences in point bounds between using
 working models with only main effects or with both main effects and interactions, as mentioned in the main text.
In fact, the sensitivity intervals from RCAL under MSM begin to include zero at $\Lambda = 20$, whereas those from CAL under MSM do not include zero until $\Lambda = 30$. Furthermore, the sensitivity intervals from RCAL under eMSM begin to include zero at $(\Lambda = 50, \delta = 0.8)$, whereas those from CAL under eMSM still do not include zero at the same $(\Lambda, \delta)$ values. 
 A possible explanation is that working models relying solely on main effects may be misspecified.

%\begin{figure}
%\centering
%\includegraphics[scale=0.6]{figure/nhanes-highdim-lin-ate-lam1.0.eps} \vspace{-.4in}
%\caption{\small
%Point bounds (x) and 90\% confidence intervals (–) on ATE under unconfoundedness $(\Lambda = 1)$, similarly as Figure \ref{fig:nhanes-highdim-lin-ate}.}
%\label{fig:nhanes-highdim-lin-ate-lam1.0}
%\end{figure}

%\begin{figure} %[H]
%\centering
%\begin{minipage}{\textwidth}
  %      \centering
   %     \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-mu-lam1.0.eps} \vspace{-.4in}
     %   \subcaption{$\Lambda = 1$}
    %\end{minipage}
    
    %\vspace{.3in}
    
  %\begin{minipage}{\textwidth}
    %    \centering
      %  \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-mu-lam10.eps} \vspace{-.4in}
       % \subcaption{$\Lambda = 10$}
    %\end{minipage}
    
    %\vspace{.3in}
    
    %\begin{minipage}{\textwidth}
      %  \centering
       % \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-mu-lam20.eps} \vspace{-.4in}
        %\subcaption{$\Lambda = 20$}
    %\end{minipage}
    
   % \vspace{.3in}
    
    %\begin{minipage}{\textwidth}
      %  \centering
        %\includegraphics[scale=0.533]{figure/nhanes-highdim-lin-mu-lam30.eps} \vspace{-.4in}
        %\subcaption{$\Lambda = 30$}
   % \end{minipage}
    
    %\vspace{.3in}
    
    %\begin{minipage}{\textwidth}
      %  \centering
       % \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-mu-lam50.eps} \vspace{-.4in}
        %\subcaption{$\Lambda = 50$}
    %\end{minipage} \vspace{-.1in}
%\caption{\small
%Point bounds (x) and 90\% confidence intervals (–) on mean blood mercury in the NHANES study, similarly as Figure \ref{fig:nhanes-highdim-lin-ate}.}
%\label{fig:nhanes-highdim-lin-mu}
%\end{figure}


\begin{figure} %[H]
\centering
\begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-lam1.0.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 1$}
    \end{minipage}
    
     \vspace{.2in}
     
  \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-lam10.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 10$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-lam20.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 20$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-lam30.eps}  \vspace{-.25in}
        \subcaption{$\Lambda = 30$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-highdim-lin-lam50.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 50$}
    \end{minipage} \vspace{-.1in}
\caption{\small
Point bounds (x) and 90\% confidence intervals (–) on mean blood mercury and ATE in the NHANES study, similarly as Figure \ref{fig:nhanes-highdim-lin-ate}.}
\label{fig:nhanes-highdim-lin}
\end{figure}



\begin{figure} %[H]
\centering
\begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-lowdim-lin-lam1.0.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 1$}
    \end{minipage}
    
     \vspace{.2in}
     
  \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-lowdim-lin-lam10.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 10$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-lowdim-lin-lam20.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 20$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-lowdim-lin-lam30.eps}  \vspace{-.25in}
        \subcaption{$\Lambda = 30$}
    \end{minipage}
    
     \vspace{.2in}
     
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[scale=0.533]{figure/nhanes-lowdim-lin-lam50.eps} \vspace{-.25in}
        \subcaption{$\Lambda = 50$}
    \end{minipage} \vspace{-.1in}
\caption{\small
Point bounds (x) and 90\% confidence intervals (–) on mean blood mercury and ATE in the NHANES study, similarly as Figure \ref{fig:nhanes-highdim-lin-ate}, but using working models with main effects only.}
\label{fig:nhanes-lowdim-lin}
\end{figure}


\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 1$, using working models with only main effects in the NHANES study.} \label{tb:nhanes-lowdim-cal-lam1.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108\\
eMSM lin &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108\\
eMSM lin &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108 &  &  0.673 &  0.108\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040\\
eMSM lin &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040\\
eMSM lin &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040 &  &  -1.093 &   0.040\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113\\
eMSM lin &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113\\
eMSM lin &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113 &  &  1.766 &  0.113\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}

\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 10$, using working models with only main effects in the NHANES study.} \label{tb:nhanes-lowdim-cal-lam10} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.290 &   0.076 &  &  -0.290 &   0.076 &  &  -0.290 &   0.076 &  &  -0.290 &   0.076\\
eMSM lin &   0.480 &   0.095 &  &   0.192 &   0.080 &  &  -0.097 &   0.074 &  &  -0.290 &   0.076\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  1.744 &  0.072 &  &  1.744 &  0.072 &  &  1.744 &  0.072 &  &  1.744 &  0.072\\
eMSM lin &  0.887 &  0.095 &  &  1.208 &  0.079 &  &  1.530 &  0.071 &  &  1.744 &  0.072\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.363 &   0.033 &  &  -1.363 &   0.033 &  &  -1.363 &   0.033 &  &  -1.363 &   0.033\\
eMSM lin &  -1.147 &   0.038 &  &  -1.228 &   0.035 &  &  -1.309 &   0.033 &  &  -1.363 &   0.033\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.677 &   0.056 &  &  -0.677 &   0.056 &  &  -0.677 &   0.056 &  &  -0.677 &   0.056\\
eMSM lin &  -1.010 &   0.041 &  &  -0.885 &   0.045 &  &  -0.760 &   0.051 &  &  -0.677 &   0.056\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  0.388 &  0.087 &  &  0.388 &  0.087 &  &  0.388 &  0.087 &  &  0.388 &  0.087\\
eMSM lin &  1.490 &  0.101 &  &  1.077 &  0.088 &  &  0.663 &  0.084 &  &  0.388 &  0.087\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.107 &  0.075 &  &  3.107 &  0.075 &  &  3.107 &  0.075 &  &  3.107 &  0.075\\
eMSM lin &  2.034 &  0.100 &  &  2.437 &  0.084 &  &  2.839 &  0.075 &  &  3.107 &  0.075\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 20$, using working models with only main effects in the NHANES study.} \label{tb:nhanes-lowdim-cal-lam20} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.414 &   0.057 &  &  -0.414 &   0.057 &  &  -0.414 &   0.057 &  &  -0.414 &   0.057\\
eMSM lin &   0.455 &   0.092 &  &   0.129 &   0.072 &  &  -0.197 &   0.059 &  &  -0.414 &   0.057\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  1.878 &  0.059 &  &  1.878 &  0.059 &  &  1.878 &  0.059 &  &  1.878 &  0.059\\
eMSM lin &  0.914 &  0.092 &  &  1.275 &  0.071 &  &  1.637 &  0.059 &  &  1.878 &  0.059\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.380 &   0.032 &  &  -1.380 &   0.032 &  &  -1.380 &   0.032 &  &  -1.380 &   0.032\\
eMSM lin &  -1.150 &   0.037 &  &  -1.236 &   0.035 &  &  -1.322 &   0.033 &  &  -1.380 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.586 &   0.068 &  &  -0.586 &   0.068 &  &  -0.586 &   0.068 &  &  -0.586 &   0.068\\
eMSM lin &  -0.991 &   0.042 &  &  -0.839 &   0.050 &  &  -0.687 &   0.060 &  &  -0.586 &   0.068\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  0.171 &  0.079 &  &  0.171 &  0.079 &  &  0.171 &  0.079 &  &  0.171 &  0.079\\
eMSM lin &  1.447 &  0.099 &  &  0.969 &  0.082 &  &  0.490 &  0.076 &  &  0.171 &  0.079\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.257 &  0.060 &  &  3.257 &  0.060 &  &  3.257 &  0.060 &  &  3.257 &  0.060\\
eMSM lin &  2.064 &  0.097 &  &  2.511 &  0.076 &  &  2.959 &  0.063 &  &  3.257 &  0.060\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 30$, using working models with only main effects in the NHANES study.} \label{tb:nhanes-lowdim-cal-lam30} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.458 &   0.050 &  &  -0.458 &   0.050 &  &  -0.458 &   0.050 &  &  -0.458 &   0.050\\
eMSM lin &   0.447 &   0.090 &  &   0.108 &   0.068 &  &  -0.232 &   0.052 &  &  -0.458 &   0.050\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  1.916 &  0.064 &  &  1.916 &  0.064 &  &  1.916 &  0.064 &  &  1.916 &  0.064\\
eMSM lin &  0.921 &  0.091 &  &  1.294 &  0.072 &  &  1.667 &  0.062 &  &  1.916 &  0.064\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.385 &   0.032 &  &  -1.385 &   0.032 &  &  -1.385 &   0.032 &  &  -1.385 &   0.032\\
eMSM lin &  -1.151 &   0.037 &  &  -1.239 &   0.034 &  &  -1.326 &   0.033 &  &  -1.385 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.534 &   0.069 &  &  -0.534 &   0.069 &  &  -0.534 &   0.069 &  &  -0.534 &   0.069\\
eMSM lin &  -0.981 &   0.042 &  &  -0.814 &   0.049 &  &  -0.646 &   0.060 &  &  -0.534 &   0.069\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  0.077 &  0.073 &  &  0.077 &  0.073 &  &  0.077 &  0.073 &  &  0.077 &  0.073\\
eMSM lin &  1.428 &  0.097 &  &  0.921 &  0.078 &  &  0.414 &  0.071 &  &  0.077 &  0.073\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.300 &  0.065 &  &  3.300 &  0.065 &  &  3.300 &  0.065 &  &  3.300 &  0.065\\
eMSM lin &  2.073 &  0.097 &  &  2.533 &  0.076 &  &  2.993 &  0.065 &  &  3.300 &  0.065\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for CAL under MSM and eMSM with $\Lambda = 50$, using working models with only main effects in the NHANES study.} \label{tb:nhanes-lowdim-cal-lam50} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.488 &   0.039 &  &  -0.488 &   0.039 &  &  -0.488 &   0.039 &  &  -0.488 &   0.039\\
eMSM lin &   0.441 &   0.090 &  &   0.092 &   0.064 &  &  -0.256 &   0.044 &  &  -0.488 &   0.039\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  1.958 &  0.077 &  &  1.958 &  0.077 &  &  1.958 &  0.077 &  &  1.958 &  0.077\\
eMSM lin &  0.930 &  0.092 &  &  1.315 &  0.075 &  &  1.701 &  0.071 &  &  1.958 &  0.077\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.389 &   0.032 &  &  -1.389 &   0.032 &  &  -1.389 &   0.032 &  &  -1.389 &   0.032\\
eMSM lin &  -1.152 &   0.037 &  &  -1.241 &   0.034 &  &  -1.329 &   0.033 &  &  -1.389 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.479 &   0.069 &  &  -0.479 &   0.069 &  &  -0.479 &   0.069 &  &  -0.479 &   0.069\\
eMSM lin &  -0.970 &   0.041 &  &  -0.786 &   0.049 &  &  -0.602 &   0.060 &  &  -0.479 &   0.069\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  -0.009 &   0.065 &  &  -0.009 &   0.065 &  &  -0.009 &   0.065 &  &  -0.009 &   0.065\\
eMSM lin &   1.411 &   0.096 &  &   0.878 &   0.075 &  &   0.346 &   0.064 &  &  -0.009 &   0.065\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.347 &  0.077 &  &  3.347 &  0.077 &  &  3.347 &  0.077 &  &  3.347 &  0.077\\
eMSM lin &  2.082 &  0.097 &  &  2.556 &  0.079 &  &  3.030 &  0.073 &  &  3.347 &  0.077\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote CAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}



\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 1$, using working models with main effects and interactions in the NHANES study.} \label{tb:nhanes-highdim-cal-lam1.0} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075\\
eMSM lin &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075\\
eMSM lin &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075 &  &  0.765 &  0.075\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038\\
eMSM lin &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038\\
eMSM lin &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038 &  &  -1.097 &   0.038\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082\\
eMSM lin &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082\\
eMSM lin &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082 &  &  1.862 &  0.082\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}

\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 10$, using working models with main effects and interactions in the NHANES study.} \label{tb:nhanes-highdim-cal-lam10} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.544 &   0.083 &  &  -0.544 &   0.083 &  &  -0.544 &   0.083 &  &  -0.544 &   0.083\\
eMSM lin &   0.495 &   0.072 &  &   0.102 &   0.071 &  &  -0.270 &   0.077 &  &  -0.544 &   0.083\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  2.099 &  0.110 &  &  2.099 &  0.110 &  &  2.099 &  0.110 &  &  2.099 &  0.110\\
eMSM lin &  1.040 &  0.075 &  &  1.441 &  0.082 &  &  1.828 &  0.096 &  &  2.099 &  0.110\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.355 &   0.032 &  &  -1.355 &   0.032 &  &  -1.355 &   0.032 &  &  -1.355 &   0.032\\
eMSM lin &  -1.145 &   0.036 &  &  -1.221 &   0.034 &  &  -1.302 &   0.033 &  &  -1.355 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.722 &   0.052 &  &  -0.722 &   0.052 &  &  -0.722 &   0.052 &  &  -0.722 &   0.052\\
eMSM lin &  -1.018 &   0.039 &  &  -0.903 &   0.043 &  &  -0.792 &   0.048 &  &  -0.722 &   0.052\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  0.178 &  0.090 &  &  0.178 &  0.090 &  &  0.178 &  0.090 &  &  0.178 &  0.090\\
eMSM lin &  1.513 &  0.079 &  &  1.005 &  0.078 &  &  0.522 &  0.084 &  &  0.178 &  0.090\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.454 &  0.113 &  &  3.454 &  0.113 &  &  3.454 &  0.113 &  &  3.454 &  0.113\\
eMSM lin &  2.185 &  0.082 &  &  2.663 &  0.087 &  &  3.130 &  0.100 &  &  3.454 &  0.113\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 20$, using working models with main effects and interactions in the NHANES study.} \label{tb:nhanes-highdim-cal-lam20} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.660 &   0.095 &  &  -0.660 &   0.095 &  &  -0.660 &   0.095 &  &  -0.660 &   0.095\\
eMSM lin &   0.469 &   0.072 &  &   0.052 &   0.074 &  &  -0.352 &   0.085 &  &  -0.660 &   0.095\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  2.329 &  0.124 &  &  2.329 &  0.124 &  &  2.329 &  0.124 &  &  2.329 &  0.124\\
eMSM lin &  1.089 &  0.076 &  &  1.546 &  0.085 &  &  2.024 &  0.108 &  &  2.329 &  0.124\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.380 &   0.032 &  &  -1.380 &   0.032 &  &  -1.380 &   0.032 &  &  -1.380 &   0.032\\
eMSM lin &  -1.153 &   0.036 &  &  -1.238 &   0.034 &  &  -1.323 &   0.033 &  &  -1.380 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.608 &   0.064 &  &  -0.608 &   0.064 &  &  -0.608 &   0.064 &  &  -0.608 &   0.064\\
eMSM lin &  -0.997 &   0.041 &  &  -0.862 &   0.048 &  &  -0.710 &   0.057 &  &  -0.608 &   0.064\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  -0.052 &   0.107 &  &  -0.052 &   0.107 &  &  -0.052 &   0.107 &  &  -0.052 &   0.107\\
eMSM lin &   1.466 &   0.079 &  &   0.914 &   0.083 &  &   0.358 &   0.096 &  &  -0.052 &   0.107\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.709 &  0.126 &  &  3.709 &  0.126 &  &  3.709 &  0.126 &  &  3.709 &  0.126\\
eMSM lin &  2.242 &  0.082 &  &  2.784 &  0.090 &  &  3.347 &  0.111 &  &  3.709 &  0.126\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 30$, using working models with main effects and interactions in the NHANES study.} \label{tb:nhanes-highdim-cal-lam30} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.808 &   0.074 &  &  -0.808 &   0.074 &  &  -0.808 &   0.074 &  &  -0.808 &   0.074\\
eMSM lin &   0.447 &   0.068 &  &  -0.016 &   0.062 &  &  -0.471 &   0.065 &  &  -0.808 &   0.074\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  2.435 &  0.118 &  &  2.435 &  0.118 &  &  2.435 &  0.118 &  &  2.435 &  0.118\\
eMSM lin &  1.108 &  0.074 &  &  1.607 &  0.082 &  &  2.103 &  0.102 &  &  2.435 &  0.118\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.385 &   0.032 &  &  -1.385 &   0.032 &  &  -1.385 &   0.032 &  &  -1.385 &   0.032\\
eMSM lin &  -1.154 &   0.036 &  &  -1.241 &   0.034 &  &  -1.327 &   0.033 &  &  -1.385 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.558 &   0.071 &  &  -0.558 &   0.071 &  &  -0.558 &   0.071 &  &  -0.558 &   0.071\\
eMSM lin &  -0.991 &   0.041 &  &  -0.837 &   0.050 &  &  -0.670 &   0.062 &  &  -0.558 &   0.071\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  -0.250 &   0.091 &  &  -0.250 &   0.091 &  &  -0.250 &   0.091 &  &  -0.250 &   0.091\\
eMSM lin &   1.438 &   0.076 &  &   0.821 &   0.074 &  &   0.199 &   0.081 &  &  -0.250 &   0.091\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  3.820 &  0.120 &  &  3.820 &  0.120 &  &  3.820 &  0.120 &  &  3.820 &  0.120\\
eMSM lin &  2.263 &  0.081 &  &  2.847 &  0.088 &  &  3.430 &  0.105 &  &  3.820 &  0.120\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}


\begin{table}
\caption{\footnotesize Point bounds and SEs for RCAL under MSM and eMSM with $\Lambda = 50$, using working models with main effects and interactions in the NHANES study.} \label{tb:nhanes-highdim-cal-lam50} \vspace{-4ex}
\begin{center}
%\renewcommand{\arraystretch}{0.9} % Reduce row height
\small
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccc}
\hline
& \multicolumn{2}{c}{$\delta = 0.2$} & & \multicolumn{2}{c}{$\delta = 0.5$} & & \multicolumn{2}{c}{$\delta = 0.8$} & & \multicolumn{2}{c}{$\delta = 1$} \\
& Bounds & SEs & & Bounds & SEs & & Bounds & SEs & & Bounds & SEs \\
\hline
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1$} \\
MSM lin &  -0.846 &   0.101 &  &  -0.846 &   0.101 &  &  -0.846 &   0.101 &  &  -0.846 &   0.101\\
eMSM lin &   0.438 &   0.070 &  &  -0.035 &   0.073 &  &  -0.499 &   0.089 &  &  -0.846 &   0.101\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1$} \\
MSM lin &  2.688 &  0.073 &  &  2.688 &  0.073 &  &  2.688 &  0.073 &  &  2.688 &  0.073\\
eMSM lin &  1.155 &  0.068 &  &  1.725 &  0.062 &  &  2.301 &  0.066 &  &  2.688 &  0.073\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^0$} \\
MSM lin &  -1.389 &   0.032 &  &  -1.389 &   0.032 &  &  -1.389 &   0.032 &  &  -1.389 &   0.032\\
eMSM lin &  -1.155 &   0.036 &  &  -1.243 &   0.034 &  &  -1.330 &   0.033 &  &  -1.389 &   0.032\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^0$} \\
MSM lin &  -0.475 &   0.079 &  &  -0.475 &   0.079 &  &  -0.475 &   0.079 &  &  -0.475 &   0.079\\
eMSM lin &  -0.987 &   0.042 &  &  -0.795 &   0.053 &  &  -0.603 &   0.068 &  &  -0.475 &   0.079\\
& \multicolumn{11}{c}{Lower bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  -0.371 &   0.118 &  &  -0.371 &   0.118 &  &  -0.371 &   0.118 &  &  -0.371 &   0.118\\
eMSM lin &   1.425 &   0.079 &  &   0.761 &   0.084 &  &   0.104 &   0.104 &  &  -0.371 &   0.118\\
& \multicolumn{11}{c}{Upper bounds and SEs for $\mu^1 - \mu^0$} \\
MSM lin &  4.076 &  0.075 &  &  4.076 &  0.075 &  &  4.076 &  0.075 &  &  4.076 &  0.075\\
eMSM lin &  2.310 &  0.075 &  &  2.967 &  0.069 &  &  3.631 &  0.070 &  &  4.076 &  0.075\\
\hline
\end{tabular}}
\end{center}
\setlength{\baselineskip}{0.5\baselineskip}
\vspace{-.15in}\noindent{\tiny
\textbf{Note}: MSM lin and eMSM lin denote RCAL under MSM and eMSM using linear outcome mean regression.}
\vspace{-.2in}
\end{table}
